An entropic generalization of Caffarelli's contraction theorem via covariance inequalities

The optimal transport map between the standard Gaussian measure and an $\alpha$-strongly log-concave probability measure is $\alpha^{-1/2}$-Lipschitz, as first observed in a celebrated theorem of Caffarelli. In this paper, we apply two classical covariance inequalities (the Brascamp-Lieb and Cram\'er-Rao inequalities) to prove a sharp bound on the Lipschitz constant of the map that arises from entropically regularized optimal transport. In the limit as the regularization tends to zero, we obtain an elegant and short proof of Caffarelli's original result. We also extend Caffarelli's theorem to the setting in which the Hessians of the log-densities of the measures are bounded by arbitrary positive definite commuting matrices.

==> commands.tex <==
\usepackage{mathtools}
\usepackage[colorlinks, linkcolor=blue,  citecolor=blue, urlcolor=blue]{hyperref}
\usepackage{autonum}
\usepackage{amssymb} %maths
\usepackage{amsthm}
\usepackage{bm}
%\usepackage{tikz}
\usepackage{url}
%----------------------------------------------
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[pdftex,dvipsnames]{xcolor}  % Coloured text etc.

%\usepackage[draft]{graphicx}
\usepackage{graphicx}
\usepackage{float}
\usepackage{subcaption}
\usepackage{multirow}
\graphicspath{{./figs/}}
%%%%%%%%%%%%%%%%%%%%



% THEOREM Environments --------------
\theoremstyle{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{principle}{Principle}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newcommand{\lemmaautorefname}{Lemma}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
\newcommand{\assumptionautorefname}{Assumption}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{claim}{Claim}
\newcommand{\claimautorefname}{Claim}


%%%%%%%%%%%%%%%%%%%%
%  Basic Commands
%%%%%%%%%%%%%%%%%%%%
%----------------------------------------------
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%% Basic Commands
\DeclareMathOperator{\grad}{\nabla}
\DeclareMathOperator{\argmin}{{argmin}}
\DeclareMathOperator{\argmax}{{argmax}}

%eigenvalues
\newcommand{\lmax}{\lambda_{\text{max}}}
\newcommand{\smax}{\sigma_{\text{max}}}
\newcommand{\smin}{\sigma_{\text{min}}}

\usepackage{adjustbox}
\usepackage{amsmath}
\usepackage{booktabs}

\usepackage{multirow, makecell}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{adjustbox}

% for custom table spacing
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%mathcals
\newcommand{\bE}{\mathbb{E}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cA}{\mathcal{A}}

%convex analysis
\newcommand{\epi}{\text{epi}}
\newcommand{\dom}{\text{dom}}
\newcommand{\sse}{\subseteq}
\newcommand{\B}{\mathbb{B}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\exR}{\R \cup \{+\infty\}}

%probability-based commands
\newcommand{\pran}[1]{\left(#1\right)}
\newcommand{\brac}[1]{\left[#1\right]}
\newcommand{\sign}[1]{\text{sign}\pran{#1}}
\newcommand{\E}[1]{\mathbb{E}\brac{#1}}
\newcommand{\Prob}[1]{\mathbb{P}\pran{#1}}
\newcommand{\qsumi}[2]{\sum_{i=#1}^{#2}}
